Delivering Ultra-Reliable Low-Latency Communications via Statistical Radio Maps

High reliability guarantees for Ultra-Reliable Low-Latency Communications (URLLC) require accurate knowledge of channel statistics, used as an input for rate selection. Exploiting the spatial consistency of channel statistics arises as a promising solution, allowing a base station to predict the propagation conditions and select the communication parameters for a new user from samples collected from previous users of the network. Based on this idea, this article provides a timely framework to exploit long-range channel spatial correlation through so-called statistical radio maps, enabling URLLC communications with given statistical guarantees. The framework is exemplified by predicting the channel capacity distribution both in a location-based radio map and in a latent space rendered by a channel chart, the latter being a localization-free approach based on channel state information (CSI). It is also shown how to use the maps to select the transmission rate in a new location that achieves a target level of reliability. Finally, several future directions and research challenges are also discussed.

==> sections/biographies.tex <==
 
\begin{IEEEbiographynophoto}{Tobias Kallehauge} is a Ph.D. student at the Connectivity Section, Electronic Systems at Aalborg University in Denmark. He received his bachelor degree in Mathematical Engineering in 2018 and a M.Sc degree in Mathematical Engineering in 2020 at Aalborg University. During his Masters's studies, he visited the University of Bremen in Germany with the European Erasmus+ program. Between 2020 and 2021, he was research assistant at the Connectivity Section, and began his Ph.D studies in 2021 with Petar Popovski as his supervisor. His current research is focused on ultra-liable low-latency communication with focus on statistical analysis and lower layer performances. 

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Pablo Ramírez-Espinosa}

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Anders E. Kalør}

\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Maxime Guillaud}
is a researcher in Huawei Technologies’ Advanced Wireless Technology Lab in Paris, France where he heads the signal and information processing group. He has over 20 years expertise in the domain of wireless communications, in both academic and industrial research environments. He received the M.Sc. degree in electrical engineering from ENSEA, Cergy, France, in 2000, and the Ph.D. degree in electrical engineering and communications from Telecom ParisTech, Paris, France, in 2005. From 2000 to 2001, he was a Research Engineer with Lucent Bell Laboratories (now Nokia), Holmdel, NJ, USA. From 2006 to 2010, he was a Senior Researcher with FTW, Vienna, Austria. From 2010 to 2014, he was a research associate with the Vienna University of Technology, Vienna. Since 2014, he has been with Huawei Technologies France. His expertise lies the physical layer of radio access networks, including transceiver algorithms, channel modeling, and modulation design.
\end{IEEEbiographynophoto}

\begin{IEEEbiographynophoto}{Petar Popovski}

\end{IEEEbiographynophoto}
